Delphi: Efficient Asynchronous Approximate Agreement for Distributed Oracles

Agreement protocols are crucial in various emerging applications, spanning from distributed (blockchains) oracles to fault-tolerant cyber-physical systems. In scenarios where sensor/oracle nodes measure a common source, maintaining output within the convex range of correct inputs, known as convex validity, is imperative. Present asynchronous convex agreement protocols employ either randomization, incurring substantial computation overhead, or approximate agreement techniques, leading to high $\mathcal{\tilde{O}}(n^3)$ communication for an $n$-node system. This paper introduces Delphi, a deterministic protocol with $\mathcal{\tilde{O}}(n^2)$ communication and minimal computation overhead. Delphi assumes that honest inputs are bounded, except with negligible probability, and integrates agreement primitives from literature with a novel weighted averaging technique. Experimental results highlight Delphi's superior performance, showcasing a significantly lower latency compared to state-of-the-art protocols. Specifically, for an $n=160$-node system, Delphi achieves an 8x and 3x improvement in latency within CPS and AWS environments, respectively.

==> 1-1-applications.tex <==
\subsection{Applications of Convergence Fairness}\label{subsec:applications}
A tradeoff between fairness and energy consumption can be utilized by in a) Collaborative machine learning, and b) Decentralized Hypothesis Testing (DHT), where the respective goals of the systems can be achieved with much lesser energy consumption using \name. 

\paragraph{Collaborative Machine Learning} We consider an $n$ node system tolerating \faults faulty nodes, where each honest node has i.i.d. training samples $(x,y)$ sampled from an underlying global function $\mathcal{F}$. The training process based on Stochastic Gradient Descent (SGD) proceeds in iterations where in each iteration, nodes locally compute gradients $g_i \forall i \in n$. The honest nodes participate in an agreement protocol to agree on the gradient $g$ that will be used in SGD. If the honest nodes use a BA protocol with only convex-hull validity and zero fairness, then the adversary can force the training process to run for more iterations by delaying convergence. The adversary does this by ensuring that in each iteration, the honest nodes agree on the value with maximum distance from the median of the set of gradients $\{g_1,g_2,\hdots,g_n\}$. When \name is used, the adversary must  choose between low fairness or higher number of rounds (and subsequently more energy). However, if the adversary chooses to delay convergence by choosing low fairness, \name takes lesser energy to terminate and therefore, consumes lower energy than any convex-hull consensus protocol. If the adversary chooses to run \name for higher number of rounds and make each training iteration costly in energy, then the resultant output of honest nodes must be fair and the training process converges faster. 

\paragraph{Decentralized Hypothesis Testing} 


==> 4-1-sec-analysis.tex <==
\section{\protocol Analysis}


==> 7-related-work.tex <==
\section{Related work}
We discuss prior works related to \name. We segment prior Asynchronous Byzantine Agreement protocols into categories based on the Validity condition of their output and the restrictions on their inputs. Many protocols were proposed with the weak Validity condition~\cite{mostefaoui2015signature,crain2020binaryba,abraham2022efficient}, which states that if all honest nodes have the same input $v$, then the output must be $v$. Binary BA protocols where nodes input only 0 or 1 offer this form of Validity. Prominent binary BA protocols~\cite{mostefaoui2015signature,crain2020binaryba,abraham2022efficient} have an \bigo{n^2} communication complexity and require \bigo{1} common coins. However, such protocols are unsuitable for applications with multi-valent inputs, where honest nodes often input multiple values. 

Many \textit{Validated} BA protocols have also been proposed with the external Validity property, where the output must be externally valid. Honest nodes in such protocols have access to a local Validity predicate that assesses the Validity of a message. An example of such a predicate is a signature verification function, which checks if the message is correctly signed. Validated Asynchronous BA(VABA)~\cite{abraham2019asymptotically} and Multi-Valued Validated BA(MVBA)~\cite{cachin2001secure,lu2020dumbo,duan2023sigfreeacs} protocols have been proposed with external Validity with a communication complexity of \bigo{\secparam n^2}, and multi-valent common coins used for electing nodes as leaders. Even though these protocols have found use in the blockchain space where a transaction's Validity can be assessed locally, such local predicates are often unavailable for real-world data like price feeds of a stock/cryptocurrency or the location of an object in an area.

Min-Max Validity enables honest nodes to agree on a value within the range of honest inputs. The popular way to achieve Min-Max Validity in asynchronous BA is to compute the Asynchronous Common Subset (ACS)~\cite{benor1994acs}, which enables agreement on a set of \highthreshold inputs. Each node then outputs the median of the ACS, which is guaranteed to be within the range of honest inputs. Concurrent ACS protocols can be classified as either being BKR-style~\cite{benor1994acs} or MVBA-style~\cite{cachin2001secure}. BKR-style ACS such as HoneyBadgerBFT~\cite{miller2016honey}, Beat~\cite{duan2018beat}, and PACE~\cite{zhang2022pace} use Reliable Broadcast(RBC) and $n$ binary BA instances, each for one node's input. However, these protocols are computationally expensive, requiring \bigo{n} common coins to terminate. They also cost \bigo{\secparam n^3} bits of communication and are notorious for their long termination times induced by the randomization for $n$ binary BA instances. Information-theoretic approaches like WaterBear do not use threshold signatures but require \bigo{exp(n)} communication to terminate. 

The MVBA-style ACS uses RBC with MVBA to overcome the high runtime of BKR-style ACS. In exchange for running $n$ binary BAs, MVBA uses a more complex multi-valent common coin for proposal election (PE), implemented using \bigo{\log(n)} binary coins~\cite{cachin2001secure}. Prior MVBA-style protocols like Dumbo2~\cite{guo2020dumbo} and SpeedingDumbo~\cite{guo2022speedingdumbo} trade computational complexity for communication efficiency and therefore use \bigo{n^2} signatures per ACS. FIN-ACS~\cite{duan2023sigfreeacs} is the most computationally efficient ACS protocol thus far, which uses RBC and a multi-valent coin for PE. FIN-ACS has an overall computational complexity of \bigo{\log(n)} coins and uses \bigo{\secparam n^3} bits, which we argue is also very expensive in our setting. 

Many approximate agreement or \approxconsensus protocols have been proposed as an alternative to the compute-intensive exact agreement protocols. Dolev \etal~\cite{dolev1986reaching} proposed the first fault-tolerant asynchronous \approxconsensus protocol with $n=5t+1$ resilience, which has \bigo{n^2} communication per round and \bigo{\log_2(\frac{\honestrange}{\epsilon})} rounds. Abraham \etal's~\cite{abraham2004approxagreement} protocol improved this resilience to 3t+1 but requires \bigo{n^3} communication per round. Many other works following Abraham \etal explored orthogonal directions like achieving \approxconsensus like gossip over a partially connected network~\cite{vaidya2012iterative}, multi-dimensional \approxconsensus~\cite{vaidya2013byzantine,mendes2015multidimensional}, and \approxconsensus with asynchronous fallback~\cite{ghinea2022syncappxaggr,ghinea2023multidimappxaggr}. However, Abraham \etal's per-round communication of \bigo{n^3} bits has not been improved so far.

==> Protocol/approx_consensus.tex <==
\begin{algorithm}
	\label{alg:early_termination}
	\caption{Cleffa: Fairness vs Runtime with optimistic early termination}
	\begin{algorithmic}[1]
		\State \textbf{INPUT}: \initialvalue{i},\honestset, \honestnodes, \secparam
		\LineComment{Honest input \initialvalue{i}, Set of all honest inputs \honestset, List of honest nodes \honestnodes, security parameter \secparam}
		\State \textbf{OUTPUT}:\outputval{i}
		\HorizontalLine
		\State \round \defeq $0$; \roundvalue{i}{0} $\leftarrow$ \initialvalue{i}
		\While{$\round < \secparam$}
		\State $\Tset{i} \leftarrow \emptyset;\Sset{i} \leftarrow \emptyset;$
		\State Invoke \rbroadcast{\roundvalue{i}{\round}}
		\State \upon terminating \rbroadcast{\roundvalue{j}{\round}}:
		\Indent
		\State $\Tset{i} \leftarrow \Tset{i} \cup j$
		\EndIndent
		\State \upon $\sizeof{\Tset{i}} == \highthreshold$:
		\Indent
		\State \textbf{call }$Gather(\Tset{i})$
		\EndIndent
		\State \upon $Gather$ delivering set \TTset{i}:
		\Indent
		\LineComment{Let $Values(\Tset{j})$ be the \highthreshold \roundvalue{k}{\round} values referenced by \Tset{j}}
		\State $\forall \Tset{j} \in \TTset{i}: \Sset{i} \leftarrow \Sset{i} \cup Median(Values(\Tset{j}))$
		\State $\roundrange{i}{\round} = \range{\Sset{i}}$ \Comment{Set range using output from gather \Sset{i}}
		\State $\Sset{i} \leftarrow Trim(\Sset{i},\sizeof{\Sset{i}}-(\highthreshold))$ \Comment{Trim $\sizeof{\Sset{i}}-(\highthreshold)$ values from each side of the set \Sset{i}}
		\EndIndent
		\If{$\roundrange{i}{\round} \leq \frac{\roundrange{i}{1}}{2^{\secparam}}$}
		\State \rbroadcast{\terminate{i}}
		\Else
		\State Invoke \commoncoin
		\EndIf
		\State \wait one of the following:
		\Indent
		\State (1) \commoncoin is delivered
		\State (2) Receiving \minthreshold \terminate{j} messages
		\EndIndent
		\If{(1) is true}
		\State $b = \commoncoin$
		\If{$b == 0$}
		\State $\roundvalue{i}{\round+1} = \minimum{\Sset{i}}$
		\ElsIf{$b == 1$}
		\State $\roundvalue{i}{\round+1} = \maximum{\Sset{i}}$
		\EndIf
		\ElsIf{(2) is true}
		\State \textbf{Terminate and output} $\outputval{i} = \roundvalue{i}{\round}$
		\EndIf
		\EndWhile
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\label{alg:verf_gather}
	\caption{Verifiable Gather protocol}
	\begin{algorithmic}[1]
		\State \textbf{INPUT}: \Tset{i},\honestnodes
		\LineComment{Honest input \Tset{i}, List of honest nodes \honestnodes}
		\State \textbf{OUTPUT}:\TTset{i}
		\HorizontalLine
		\State $\TTset{i} \leftarrow \emptyset;\Hset{i1} \leftarrow \emptyset; \Hset{i2} \leftarrow \emptyset; \Hset{i3} \leftarrow \emptyset;$
		\State Invoke \rbroadcast{\gathermsg{1}{\Tset{i}}}
		\State \upon terminating \rbroadcast{\gathermsg{1}{\Tset{j}}} and terminating \rbroadcast{\roundvalue{k}{\round}} $\forall k \in \Tset{j}$:
		\Indent
		\State $\TTset{i} \leftarrow \TTset{i} \cup \Tset{j}$
		\State $\Hset{i2} \leftarrow \Hset{i2} \cup j$
		\EndIndent
		%\LineComment{Each value in \Sset{i} is a safe value: all values from faulty nodes in \Sset{i} must be within the range of honest values}
		\State \upon $\sizeof{\Hset{i2}} == \highthreshold$: \Indent
		\State \sendall{\gathermsg{2}{\Hset{i2}}}
		\EndIndent
		\State \upon receiving \gathermsg{2}{\Hset{j2}} and $\sizeof{\Hset{j2}}\geq\highthreshold$: 
		\Indent
		\State \upon $\Hset{j2} \subseteq \Hset{i2}$:
		\Indent
		\State $\Hset{i3} \leftarrow \Hset{i3} \cup j$
		\If{$\sizeof{\Hset{i3}}=\highthreshold$}
		\State \sendall{\gathermsg{3}{\Hset{i3}}}
		\EndIf
		\EndIndent
		\EndIndent
		\State \upon receiving \gathermsg{3}{\Hset{j3}} and $\sizeof{\Hset{j3}} \geq \highthreshold$:
		\Indent
		\State \upon $\Hset{j3}\subseteq \Hset{i3}$:
		\Indent
		\State $\Hset{i3} \leftarrow \Hset{i3} \cup j$
		\EndIndent
		\EndIndent
		\State \upon $\sizeof{\Hset{i3}}=\highthreshold$: 
		\Indent
		\State \textbf{Output: }\TTset{i}
		\EndIndent
	\end{algorithmic}
\end{algorithm}

==> Protocol/aux.tex <==
\LineComment{Procedure to split interval into smaller ones}
\State{}\textbf{helper method }\decompose($\binaastateval{a}{b}{l}$)\label{algline:decompose}:
\Indent
\If{$\exists \interval{a}{b}{l}\in self.intervals: a<x<b$}
\State{} $\{\interval{a}{x}{l},\interval{x}{b}{l}\}\leftarrow \interval{a}{b}{l}$
\State{} $self.intervals\leftarrow self.intervals\setminus \interval{a}{b}{l}$ 
\State{} $self.intervals\leftarrow self.intervals\cup \{\interval{a}{x}{l},\interval{x}{b}{l}\}$
\EndIf{}
\If{$\exists \interval{a}{b}{l}\in self.intervals: a<y<b$}
\State $\{\interval{a}{y}{l},\interval{y}{b}{l}\}\leftarrow \interval{a}{b}{l}$
\State{} $self.intervals\leftarrow self.intervals\setminus \interval{a}{b}{l}$ 
\State{} $self.intervals\leftarrow self.intervals\cup \{\interval{a}{y}{l},\interval{y}{b}{l}\}$
\EndIf{}
\EndIndent

\protocolrbc\footnoteAppxAggr{}
%&
%async.
%&
%1/3
%&
%D
&
\bigo{|V|n^2\log(\frac{n\honestrange}{\epsilon})+n^3}
%&
%\bigo{n^3}
&
\bigo{\log(\frac{n\honestrange}{\epsilon})}
&
0
&
0
%&
%\bigo{1}
&
$[m-\honestrange,M+\honestrange]$
%&
%None
&
Auth.\ channels
\\


\State{}\textbf{helper method }\coalesce(\levelencap)$\to\levelencap$:\label{algline:coalesce}
\LineComment{This condition is true when all honest inputs $\oracleinput{i}\in\interval{j}{j+1}{l}$}
\Indent{}
\State{} Check if only two consecutive checkpoints \intervalmidpoint{\checkpointindex}{}{l} and \intervalmidpoint{\checkpointindex+1}{}{l} has weight 1 and remaining others have weight 0 at level $l$. Check if this condition is true for all levels $l'$ until $\levelmax$ for two closest checkpoints \intervalmidpoint{z}{}{l'} \intervalmidpoint{z+1}{}{l'} to \intervalmidpoint{\checkpointindex}{}{l} and \intervalmidpoint{\checkpointindex+1}{}{l}
\LineComment{Replace all weights from level $l$ to \levelmax{} with a constant sized value}
\State{}$\levelencap{}[l^{*}]\leftarrow\{\} \forall l^{*}\in\{l,\hdots,\levelmax\}$
\State{}$\levelencap[l]$ $\leftarrow \levelencap[l] \cup \multlevel{c\overshoot{l}}{l}{\levelmax}{r}$\label{algline:replace_msgs_coalesce}
\State{}\textbf{return } \levelencap{}
\EndIndent{}

\State{}\textbf{helper method }\expand(\levelencap)$\to\levelencap$:
\Indent{}
\If{$\exists \multlevel{m}{l}{\levelmax}{r} \in \levelencap$}
\State{} \levelencap$\leftarrow \levelencap \setminus \multlevel{m}{l}{\levelmax}{r}$
\State{} Insert level messages \levelmsgwrapper{\levelmsg}{l} for $\{l,\hdots,\levelmax\}$ into \levelencap, where each \levelmsg{} contains weight 1 for interval with $m$ and 0 for all others.
\EndIf{}
\State{} \textbf{return } \levelencap{}
\EndIndent{}

\begin{definition}\akhil{We can remove this primitive if needed for space}
	A crusader agreement protocol $\Pi_{CA}$ for $n$ nodes where node $i$ inputs \oracleinput{i}$\in\{0,1\}$ must have the following guarantees.
	\adithya{\emph{amongst} is rarely used. Use among. In this case \emph{for} makes more sense.}
	% https://paperpal.com/blog/academic-writing-guides/language-grammar/among-vs-amongst#:~:text=“Amongst”%20is%20a%20preposition%20used,generally%20limited%20to%20specific%20contexts.
	\begin{itemize}
		\item \textbf{Termination}: All non-faulty nodes must eventually terminate and output a value.
		\item \textbf{Validity}: If all non-faulty nodes input the same value, then it must be the output.
		\item \textbf{Agreement}: If two non-faulty nodes decide $x$ and $y$, then either $x=y$ or at least one of the values is \bottom.
	\end{itemize}
	\adithya{This definition is incorrect. See latex source file for a commented reference.}
	% https://decentralizedthoughts.github.io/2022-04-05-aa-part-four-CA-and-BCA/
\end{definition}

==> Protocol/avss.tex <==
%Commented out
\begin{comment}
\rebox
\begin{figure}[!tbp]
    \label{protocol:RZ}
    \caption{\protocol{RZ}}
    \begin{flushleft}
        We assume that the \textit{Setup($1^k,n-t$)} phase has already been run and every honest node has a trusted setup $SP$ before beginning the protocol.  Every honest node follows the following steps: 
        \begin{enumerate}[wide]
            \item \textbf{Secret sharing phase}: Every node begins the protocol with \initialvalue{}. An honest node $i$ shares \initialvalue{i} by invoking the function \secretshare{\initialvalue{i}}. 
            \item \textbf{Collect secrets and commitments}: An honest node $i$ keeps track of secret sharing instances using variable \secretsharinginst{i}{j}, $\forall j \in \noderange{1}{n}$. If node $i$ completes the AVSS protocol started by node $j$, it sets $\secretsharinginst{i}{j} = 1$ and adds the commitment \commitment{j} to its commitment set \commitmentset{i}. 
            \item \textbf{Create and \rbroadcast{i}{\report{i}{j}}}: If an honest node $i$ completes the AVSS protocol of another node $j$, it creates a report $\report{i}{j} = \langle\commitment{j},\sign{i}{\commitment{j}}\rangle.$ The node reliably broadcasts \report{i}{j} by invoking \rbroadcast{i}{\report{i}{j}}. 
            \item \textbf{Wait for \highthreshold stable witnesses}: If an honest node $i$ invokes \rdeliver{i}{\report{j}{k}}, it adds \report{j}{k} to its report set \reportset{i}{j}.
            \begin{gather}
                \textit{On }\rdeliver{i}{\report{j}{k}}, \reportset{i}{j} = \reportset{i}{j} \cup \report{j}{k}
            \end{gather}
            As described previously, a stable witness to node $i$ is any node $j$ whose first \highthreshold stable secrets are stable at node $i$.
            \begin{gather}
                \textit{On } |\commitmentset{i} \cap \reportset{i}{j}| = \highthreshold: \rwitnesses{i} = \rwitnesses{i} \cup j
            \end{gather}
            The node $i$ waits until accepting 
            The honest node waits until:
            \begin{gather}
                |W_i| = \highthreshold
            \end{gather}
            \item \textbf{Start reconstruction for all accepted messages}: After receiving \highthreshold stable witnesses, an honest node $i$ reveals its share of the secrets it received reliably. 
            \begin{gather}
                (|W_i| = \highthreshold) \Rightarrow (\forall j: \secretsharinginst{i}{j}=1, \reconstructsecret{i}{\secretsharinginst{i}{j}})
            \end{gather}
            \item \textbf{Wait until knowing all secrets received}: An honest node $i$ will wait until all secrets it received are opened. It adds every revealed secret to its \valueset{i} and applies the reduce function \reduce{\valueset{i}}{\faults}.
            \begin{gather}
                \initialvalue{i} = \reduce{\valueset{i}}{f}
            \end{gather}
            \item \textbf{Run \protocol{WT} with \initialvalue{i}}: The honest nodes will run \protocol{WT} on updated values \initialvalue{i}. 
        \end{enumerate}
    \end{flushleft}
\end{figure}
\unbox
\begin{algorithm*}
\begin{multicols}{2}
\small
\label{alg:rz}
\caption{Protocol for Asynchronous predicate diffusion}
\SetKwComment{Comment}{}{}
\Comment{As honest node $i$ participating in the protocol.}\
INPUT: \hmessage{i}\;
\algrule
	\setcounter{AlgoLine}{100}
	\Comment{// SHARING PHASE}\
	\avsssh(\hmessage{i})\;
	\algrule
	\setcounter{AlgoLine}{200}
	\Comment{// WAIT FOR \highthreshold CORROBORATORS}
	$\rsreport{i}{j} \leftarrow \{\} \forall j \in \noderange{1}{n}; \corroborators{i} \leftarrow \{\}$\;
	\While{$|\corroborators{i}| < \highthreshold$}{
		\Comment{// WAIT FOR SECRET SHARES, SEND REPORTS,}
		\Comment{// AND WAIT FOR \highthreshold STABLE SECRETS}
		% got n-f stable witnesses?
		$\secrets{i} \leftarrow \{\}; \reportset{i}{j} \leftarrow \{\} \forall j \in \noderange{1}{n}; \stablesecrets{i} \leftarrow \{\}$\\
		\textbf{upon} termination of $j$th AVSS:\\
		\tab Let \secret{j}{i} be the share of node $i$ for $j^{th}$ AVSS.\\
		\tab $\secrets{i} \leftarrow \secrets{i} \cup \secret{j}{i}$\\
		\tab \Comment{// Create and SendAll Report}
		% Remove signatures from everything, authenticated channels are enough, signatures are not needed. 
		\tab $\report{i}{j} \leftarrow \langle j, i \rangle$\\
		\tab \fifosendall{i}{\report{i}{j}}\\
		\label{alg:step:fiforsendall}
		\textbf{upon} FIFO receiving \report{j}{k}:\\
		\tab $\reportset{i}{k} \leftarrow \reportset{i}{k} \cup \report{j}{k}$\\
		\tab \Comment{// Add to stable secret list after}
		\tab \Comment{// receiving \threshold+\faults reports of $k$}
		\tab \textbf{upon} $|\reportset{i}{k}| \ge \threshold+\faults$:\\
		\tab \tab $\stablesecrets{i} \leftarrow \stablesecrets{i} \cup j$\\
		\Comment{// Broadcast stable secret list after}
		\Comment{// receiving \highthreshold stable secrets}
		\label{algstep:stable_secrets}
		\textbf{upon} $|\stablesecrets{i}| = \highthreshold$:\\
		\tab \attestation{i}:=\stablesecrets{i}\;
		\tab $\rbroadcast{i}{\langle\attestation{i}\rangle}$\;
		\textbf{upon} reliably receiving \attestation{j}:\\
		\tab $\rsreport{i}{j} \leftarrow \attestation{j}$\;
		\Comment{// CHECK FOR CORROBORATORS}
		\If{$\rsreport{i}{j} \neq \emptyset$}{
			\Comment{// Node $i$ must receive \highthreshold}
			\Comment{// reports for every $k$ in \rsreport{i}{j}}
			\If{$|\reportset{i}{k}| \ge \highthreshold \forall k \in \rsreport{i}{j}$}{
				$\corroborators{i}\leftarrow\corroborators{i}\cup j$ 
			}
		}
	}
	\Comment{// SECRET RECONSTRUCTION PHASE}
	\setcounter{AlgoLine}{300}
	\Comment{// Start reconstruction for all terminated AVSS}
	\For{$\secret{j}{i} \in \secrets{i}$}{
		\avssrec(\secret{j}{i})\;
	}
	\label{algstep:secret_recovery}
	\Comment{// Wait until reconstructing secrets that received  \threshold+\faults REPORTS}
	\For{$j : |\reportset{i}{j}|\ge \highthreshold$}{
		\valueset{i} $\leftarrow$ \valueset{i} $\cup$ 
		\avssrec(\secret{j}{i})
	}
	OUTPUT: \valueset{i}
	\algrule
	%\initialvalue{i} $\leftarrow$ \reduce{i}{\valueset{i}}\;
	%\protocol{WT}(\initialvalue{i})\;
	\end{multicols}
\end{algorithm*}
%\begin{multicols}{2}
	\begin{algorithm}
		\caption{\protocol{APD}: Protocol for Asynchronous predicate diffusion}
		\small
		\label{alg:apd}
		\begin{algorithmic}[1]
		\State \textbf{INPUT}: \hmessage{i}\Comment{As honest node $i$ participating in the protocol.}
		\State // For $n=3\faults+1$ settings, we use ACSS scheme proposed in \cite{das2021add} with $t=\minthreshold$. For $n=4\faults+1$, we use the AVSS scheme proposed by \cite{das2021add} with $t=\minthreshold$.
		\setcounter{ALG@line}{100}
		\State \avsssh(\hmessage{i})\Comment{ SHARING PHASE START}
		%\Comment{// WAIT FOR \highthreshold CORROBORATORS}\\
		\State $\rsreport{i}{j} \leftarrow \{\} \forall j \in \noderange{1}{n}; \corroborators{i} \leftarrow \{\}$\;
		\While{$|\corroborators{i}| < \highthreshold$} \Comment{Wait for \highthreshold Corroborators}
			\State{// WAIT FOR SECRET SHARES, SEND REPORTS, AND WAIT FOR \highthreshold STABLE SECRETS}
			% got n-f stable witnesses?
			\State $\secrets{i} \leftarrow \{\}; \reportset{i}{j} \leftarrow \{\} \forall j \in \noderange{1}{n}; \stablesecrets{i} \leftarrow \{\}$
			\State \textbf{upon} termination of $j$th AVSS:
			\State \tab Let \secret{j}{i} be the share of node $i$ for $j^{th}$ AVSS.
			\State \tab $\secrets{i} \leftarrow \secrets{i} \cup \secret{j}{i}$
			% Remove signatures from everything, authenticated channels are enough, signatures are not needed. 
			\State \tab $\report{i}{j} \leftarrow \langle j, i \rangle$ \Comment{Create and SendAll Report}
			\State \tab \sendall{i}{\report{i}{j}} 
			\label{alg:step:fiforsendall}
			\State \textbf{upon} Receiving \report{j}{k}:
			\label{alg:step:receive}
			\State \tab $\reportset{i}{k} \leftarrow \reportset{i}{k} \cup \report{j}{k}$
			\State \tab \textbf{upon} $|\reportset{i}{k}| \ge \threshold+\faults$: \Comment{Add to stable secret list after receiving \threshold+\faults reports of $k$}
			\State \tab \tab $\stablesecrets{i} \leftarrow \stablesecrets{i} \cup j$
			
			\label{algstep:stable_secrets}
			\State \textbf{upon} $|\stablesecrets{i}| = \highthreshold$: \Comment{RBroadcast attestation after receiving \highthreshold stable secrets}
			\State \tab \attestation{i}:=\stablesecrets{i}\;
			\State \tab $\rbroadcast{i}{\langle\attestation{i}\rangle}$\;
			\label{algstep:rbattestation}
			\State \textbf{upon} reliably receiving \attestation{j}:
			\State \tab $\rsreport{i}{j} \leftarrow \attestation{j}$\;
			\If{$\rsreport{i}{j} \neq \emptyset$} \Comment{Check for corroborators}
				%\Comment{// Node $i$ must receive \highthreshold REPORTS for every $k$ in \rsreport{i}{j}}\\
				%\Comment{// reports for every $k$ in \rsreport{i}{j}}\\
				\If{$|\reportset{i}{k}| \ge \highthreshold \forall k \in \rsreport{i}{j}$} \Comment{Node $i$ must receive \highthreshold REPORTS for every $k$ in \rsreport{i}{j}}
					\State $\corroborators{i}\leftarrow\corroborators{i}\cup j$ 
				\EndIf
			\EndIf
		\EndWhile \Comment{SHARING PHASE END}
		\State \hrulefill
		\setcounter{ALG@line}{200}
		\For{$\secret{j}{i} \in \secrets{i}$} \Comment{SECRET RECONSTRUCTION PHASE START}
			\State \avssrec(\secret{j}{i}) \Comment{Start reconstruction for all terminated AVSS}
		\EndFor
		\label{algstep:secret_recovery}
		\For{$j : |\reportset{i}{j}|\ge \highthreshold$} \Comment{Wait until reconstructing secrets that received  \threshold+\faults REPORTS}
			\State \valueset{i} $\leftarrow$ \valueset{i} $\cup$ 
			\avssrec(\secret{j}{i})
		\EndFor \Comment{RECONSTRUCTION PHASE END}
		\State \textbf{OUTPUT}: \valueset{i}
		%\initialvalue{i} $\leftarrow$ \reduce{i}{\valueset{i}}\;
		%\protocol{WT}(\initialvalue{i})\;
		\end{algorithmic}
	\end{algorithm}
\begin{algorithm}
	\caption{\reduce{S}{\faults} - Set reduction function \cite{abraham2004approxagreement}}\label{alg:reduce_proc}
	\begin{algorithmic}[1]
		\State \textbf{INPUT}: S,\faults
		\State The function $\trim{S}{\faults}$ trims out $\faults$ values from each end of the set $S$.
		\State $S \leftarrow \trim{\sort{S}}{\faults}$
		\State $\textit{out} \leftarrow \frac{\minimum{S} + \maximum{S}}{2}$
		\State \textbf{OUTPUT}: \textit{out}
	\end{algorithmic}
\end{algorithm}
\end{comment}
\begin{algorithm}
	\caption{\protocolapd: Protocol for Asynchronous predicate diffusion}
	\small
	\label{alg:apd}
	\begin{algorithmic}[1]
		\State \textbf{INPUT}: \hmessage{i} $\in$ $\mathcal{M}$
		\State Public parameters:\pk{j} for j $\in \noderange{1}{n}$
		\State \textbf{OUTPUT}: \outputset{i}
		\HorizontalLine
		\LineComment{SHARING PHASE}
		\setcounter{ALG@line}{100}
		\State \avsssh(\hmessage{i})
		\label{algline:acss}
		\HorizontalLine
		\State \secrets{i}  =\setop{}; \reportset{i}{j}=\setop{} for j $\in \noderange{1}{n}$
		\label{algline:secret_initialization}
		\State \stablesecrets{i} = \setop{}; \rsreport{i}{j} = \setop{} for j $\in \noderange{1}{n}$
		\label{algline:stable_secret_initialization}
		\State \corroborators{i} = \setop{}, \secretshares{i}{j} = \setop{} for j $\in \noderange{1}{n}$
		\label{algline:corroborator_set}
		\State \upon termination of $j$th \avsssh(\hmessage{j}):
		\State \tab $\secrets{i} = \secrets{i}\cup \setop{\secretshare{j}{i}}$
		\State \tab \sendall{\report{i}{j}} \Comment{Create and SendAll Report}
		\label{algline:sendall}
		\State \upon receiving \report{j}{k}:
		\State \tab \reportset{i}{k} = \reportset{i}{k} $\cup$ $\setop{j}$
		\State \upon \sizeofset{\reportset{1}{j}} $\geq 2\faults+1$ and terminating $j$'s \avsssh(\hmessage{j}):
		\label{algline:condition_ss}
		\State \tab \stablesecrets{i} = \stablesecrets{i} $\cup$ \setop{j}
		\label{algline:stable_secrets}
		\State \upon \sizeofset{\stablesecrets{i}} = \highthreshold for the first time:
		\State \tab \rbroadcast{}{\attestation{\stablesecrets{i}}} \Comment{\rbroadcast{}{} attestation after receiving \highthreshold stable secrets}
		\label{algline:attestation_broadcast}
		\State \upon \rdeliver{\attestation{\stablesecrets{j}}}:
		\State \tab \reportset{i}{j} = \stablesecrets{j}
		\State \upon \reportset{i}{j} such that $\forall k \in \reportset{i}{j}: k \in \stablesecrets{i}$: \Comment{Check for corroborators}
		\State \tab \corroborators{i} = \corroborators{i} $\cup$ \setop{j}
		\State \upon \sizeofset{\corroborators{i}} =\highthreshold: \Comment{Wait for \highthreshold corroborators}
		\State \tab $\forall \secretshare{j}{i} \in \secrets{i}: \sendall{\secretshare{j}{i}}$
		\label{algline:broadcast_ss}
		\HorizontalLine
		\LineComment{RECONSTRUCTION PHASE}
		\setcounter{ALG@line}{200}
		\State \verifiedsecretshares{i}{j} = \setop{} $\forall j \in \noderange{1}{n}$
		\State \outputset{i} = \setop{};
		\State \upon receiving \secretshare{j}{k}:
		\State \tab \secretshares{i}{j} = \secretshares{i}{j} $\cup$ \secretshare{j}{k}
		\State \tab \upon j $\in$ \stablesecrets{i} and verifying share \secretshare{j}{k}: \Comment{Verifying shares only possible after terminating $j$'s\avsssh}
		\State \tab \tab \verifiedsecretshares{i}{j} = \verifiedsecretshares{i}{j} $\cup$ \secretshare{j}{k}
		\State \upon \sizeofset{\verifiedsecretshares{i}{j}}$\geq$ \minthreshold:
		\State \tab \outputset{i} = \outputset{i} $\cup$ \setop{\avssrec(\verifiedsecretshares{i}{j})}
		\label{algstep:secret_recovery}
		\State \upon reconstructing all secrets shared by $j \in \stablesecrets{i}$: 
		\label{algline:wait_condition}
		\State \tab\textbf{OUTPUT}: \outputset{i}
	\end{algorithmic}
\end{algorithm}
%\end{multicols}

==> Protocol/binary_appx_consensus.tex <==
\begin{algorithm}
	\label{alg:bin_appx_consensus}
	\caption{Approximate Agreement Protocol with binary inputs}
	\begin{algorithmic}[1]
		\State \textbf{INPUT}: \initialvalue{i},\aaprecision
		\LineComment{Honest input $\initialvalue{i} \in \{c_0,c_1\}$}
		\Comment{Honest nodes' inputs are binary.}
		\State \textbf{OUTPUT}:\outputval{i}
		\HorizontalLine
		\State $r_t$ \defeq $\log_{2}(\frac{c_1-c_0}{\aaprecision})$; \roundvalue{i}{1} \defeq \initialvalue{i}
		\State $\round \defeq 1; \mathcal{R} \leftarrow \emptyset$
		\State $\terminate \defeq false$
		\While{true}
		\State $\Tset{i} \leftarrow \{\}$
		\If{$\round < r_t$}
		\State $SendAll(\langle ECHO,\roundvalue{i}{\round},\round\rangle)$
		\State $\round = \round+1$
		\ElsIf{$\round == r_t$}
		\State \text{Terminate and return } $\outputval{i} = \roundvalue{i}{\round}$
		\EndIf
		\State \upon receiving $\faults+1$ $\langle ECHO,V',\round \rangle$ messages for $V' \neq \roundvalue{i}{\round}$:
		\State \tab $SendAll(\langle ECHO, V',\round\rangle)$
		\State \upon receiving $2\faults+1$ $\langle ECHO,V,\round\rangle$ messages:
		\State \tab $\Tset{i} \leftarrow \Tset{i} \cup V$
		\Indent
		\If{ECHO2 not sent previously}:
		\State $SendAll(\langle ECHO2, V, \round\rangle)$
		\EndIf
		\EndIndent
		\State \textbf{wait until one of the following conditions are true:}
		\Indent
		\State (1) $\sizeof{\Tset{i}} == 2$ [OR]
		\State (2) until receiving $2f+1$ $\langle ECHO2,V\rangle$ messages for value $V$
		\If{(1) is true}
		\State \tab $\roundvalue{i}{\round+1} = \frac{\Tset{i}[0]+\Tset{i}[1]}{2}$
		\ElsIf{(2) is true}
		\State \tab $\roundvalue{i}{\round+1} = V$
		\EndIf
		\EndIndent
		\EndWhile 
	\end{algorithmic}
\end{algorithm}
\begin{comment}
	\begin{algorithm}
		\label{alg:bin_appx_consensus_rnd_est}
		\caption{EstimateRounds}
		\begin{algorithmic}[1]
			\State \textbf{INPUT}: \initialvalue{i},\aaprecision, \honestnodes
			\LineComment{Honest input $\initialvalue{i} \in \{c_0,c_1\}$, List of honest nodes \honestnodes}
			\Comment{Honest nodes' inputs are binary. Honest nodes need not necessarily know $c_0$ and $c_1$.}
			\State \textbf{OUTPUT}:\outputval{i}
			\HorizontalLine
			\State $\Tset{i} \leftarrow \set{\initialvalue{i}},\Sset{i} \leftarrow \{\}, \witnesses{i} \leftarrow \{\}$
			\State $SendAll(\langle ECHO,\initialvalue{i}\rangle)$
			\State \upon receiving $\faults+1$ $\langle ECHO,V' \rangle$ messages for $V' \neq \initialvalue{i}$:
			\State \tab $\Tset{i}\leftarrow \Tset{i} \cup V'$
			\State \tab $SendAll(\langle ECHO, V'\rangle)$
			\State \upon receiving $2\faults+1$ $\langle ECHO,V\rangle$ messages:
			\State \tab $\Sset{i} \leftarrow \Sset{i} \cup V$
			\State \tab $SendAll(\langle ECHO2, V\rangle)$
			\State \textbf{wait until one of the following conditions are true:}
			\Indent
			\State (1) $\sizeof{\Sset{i}} == 2$ [OR]
			\State (2) until receiving $2f+1$ $\langle ECHO2,V\rangle$ messages for value $V$
			\If{(1) is true}
			\State $\roundvalue{i}{1} = \frac{\Sset{i}[0]+\Sset{i}[1]}{2}$
			\ElsIf{(2) is true}
			\State $\roundvalue{i}{1} = V$
			\EndIf
			\EndIndent
			\Comment{Round Estimation}
			\State $SendAll(\langle RE,\Tset{i}\rangle)$
			\State \upon receiving $\langle RE, \Tset{j}\rangle$ message and $\forall V \in \Tset{j} : V \in \Tset{i}$:
			\Indent
			\State $\witnesses{i}\leftarrow\witnesses{i} \cup j$
			\EndIndent
			\State \upon $\sizeof{\witnesses{i}}==\highthreshold$:
			\Indent
			\If{$\sizeof{\Tset{i}}==1$}
			\State $r_t$ \defeq 1
			\ElsIf{$\sizeof{\Tset{i}}==2$}
			\State $r_t$ \defeq $\log_{2}(\frac{\sizeof{\Tset{i}[0]-\Tset{i}[1]}}{\aaprecision})$
			\EndIf
			\EndIndent
			\State \textbf{return }$\langle \roundvalue{i}{1},r_t\rangle$
		\end{algorithmic}
	\end{algorithm}
\end{comment}

==> Protocol/hash_ss.tex <==
\begin{algorithm*}
	\small
	\caption{\bawvssprot: Batch Asynchronous Weak Verifiable Secret Sharing (\bawss)}
	\label{alg:bawss}
	\begin{algorithmic}[1]
		\begin{multicols}{2}
		\State \textbf{INPUT}: \nodeset,\rbcprot,\secrets{d} \Comment{\rbcprot: RBC protocol,\secrets{d}: secrets to share}
		\HorizontalLine
		\State Protocol \bavsssh{d}{\secrets{d}}:
		\State \upon receiving (ID.d,in,{\sc{share}},\secrets{d}):\Comment{As a dealer}
		\Indent
		\LineComment{Sample \sizeof{\secrets{d}} nonces from a domain $\domain'$ at least twice the \hashfunc's output range}
		$\nonce_d[i] \leftarrow Random(\domain') \forall i\in\{1,\hdots,\sizeof{\secrets{d}}\}$
		\LineComment{Use Shamir's SS scheme to create shares for secrets in \secrets{d}, $\nonce_d[i]$}
		\State $\secretshares{d}{i} \leftarrow$\shamir{\secrets{d}[i]}{n}{\faults} $\forall i \in \{1,\hdots,\sizeof{\secrets{d}}\}$
		\State $\nonceshares{d}{i} \leftarrow$\shamir{$\nonce_d[i]$}{n}{\faults} $\forall i \in \{1,\hdots,\sizeof{\secrets{d}}\}$\label{algline:bawss:shamir_create}
		\LineComment{Compute Commitments}
		\State $\commarr{d}{i} \leftarrow \tup{\hashfunc(\nonceshares{d}{i}[0],\secretshares{d}{i}[0]),\hdots,\hashfunc(\nonceshares{d}{n}[0],\secretshares{d}{i}[n])} \forall i \in \{1,\hdots,\sizeof{\secrets{d}}\} $ 
		\LineComment{Compute Merkle Trees}
		\State $M_d[i] = $ {\sc{Merkle}}(\commarr{d}{i}) $\forall i \in \{1,\hdots,\sizeof{\secrets{d}}\}$ 
		\State $\rootvec{d}\leftarrow\setop{M_d[0].\text{{\sc{Root}}},\hdots,M_d[k].\text{{\sc{Root}}}}$
		\State $\nodeshares{d}{j}[i] \leftarrow \tup{\secretshares{d}{i}[j],\nonceshares{d}{i}[j],M_d[i].{\text{\sc{Proof}}(j)}} \forall i\in\{1,\hdots,\sizeof{\secrets{d}}\},\forall j \in \{1,\hdots,n\}$\label{algline:bawss:node_share_vector}
		\LineComment{Send shares to all nodes}
		\For{$j \in \{1,\hdots,n\}$}
		\State Send "ID.d, {\sc{share}}, \nodeshares{d}{j}" to node \node{j}
		\EndFor
		\LineComment{Reliably Broadcast root vector}
		\State Invoke \rbroadcast{\rootvec{d}}\label{algline:bawss:rbc}
		\EndIndent 
	\LineComment{As a participant}\\
		\upon receiving "ID.d,{\sc{share}},\nodeshares{d}{j}" and \rbcinit{\rootvec{d}} from dealer \node{d}:
		\Indent
		\LineComment{Verify commitments and participate in \rbcprot if all pass}
		\If{{\sc{Merkle.Verify}($\rootvec{d}[i]$,$\nodeshares{d}{j}[i].${\sc{share}},$\nodeshares{d}{j}[i]$.{\sc{proof}})} $= 1 \forall i \in \{1,\hdots,\sizeof{\secrets{d}}\}$}
			\State Send ECHO messages in \node{d}'s RBC protocol \rbcprot\label{algline:part_rbc}\label{algline:bawss:verify_comm}
		\EndIf
		\EndIndent
		\State \upon invoking \rdeliver{\rootvec{d}} with share:
		\Indent
		\State \textbf{output} (ID.d,out,{\sc{share}},\rootvec{d})
		\EndIndent
		\State \upon invoking \rdeliver{\rootvec{d}} with no share:
		\Indent
		\State \textbf{output} (ID.d,out,{\sc{no-share}},\rootvec{d})
		\EndIndent
		\HorizontalLine
		\setcounter{ALG@line}{0}
		\State Protocol \bavssrec{d}{i}:
		\State $\tmpsecretshares{d}{i}\leftarrow\emptyset$
		\State \upon receiving (ID.d,in,{\sc{recon}},$i$): 
		\Indent
		\If{terminated with {\sc{share}}}
		\For{$j \in \{1,\hdots,n\}$}
		\State Send "ID.d, {\sc{recon}},\nodeshares{j}{i}" to node \node{j}\label{algline:bawss:rec_send}
		\EndFor
		\EndIf
		\EndIndent
		\State \upon receiving (ID.d,{\sc{recon}},$\nodeshares{d}{m}[i]$) from node \node{m}:
		\Indent
		\If{{\sc{Merkle.Verify}}($\rootvec{d}[i]$,$\nodeshares{d}{m}[i].${\sc{share}},$\nodeshares{d}{m}[i]$.{\sc{proof}}) $= 1$}\label{algline:verf_proof}
		\State $\tmpsecretshares{d}{i} \leftarrow\tmpsecretshares{d}{i} \cup \langle m,\nodeshares{d}{m}[i]\rangle$
		\EndIf
		\EndIndent
		\upon {$\sizeof{\tmpsecretshares{j}{i}} \geq \minthreshold$}
		\Indent
		\LineComment{Combine shares and reverify root vector commitment}
		\State $\secretshares{d}{i},\nonceshares{d}{i} \leftarrow$ \shamircomb{\tmpsecretshares{d}{i}}{n}{\faults}\label{algline:bawss:recon}
		\State $\commarr{d}{i} \leftarrow \tup{\hashfunc(\nonceshares{d}{i}[0],\secretshares{d}{i}[0]),\hdots,\hashfunc(\nonceshares{d}{i}[n],\secretshares{d}{i}[n])} \forall i \in \{1,\hdots,\sizeof{\secrets{d}}\}$
		\If{{\sc{Merkle}}(\commarr{d}{i}).{{\sc{Root}}} = \rootvec{i}}
		\State \textbf{output} (ID.d,out,{\sc{reconstructed}},$\secretshares{d}{i}[0]$,$i$)
		\Else
		\State \textbf{output} (ID.d,out,{\sc{reconstructed}},\bottom,$i$)
		\EndIf 
		\EndIndent
		\end{multicols}
	\end{algorithmic}
\end{algorithm*}

==> Protocol/interval.tex <==
\begin{algorithm}
  \small
  \caption{Checkpoint}%
  \label{alg:interval}
  \begin{algorithmic}[1]
    \Statex{} {\color{myorange}\(\triangleright\) \textrm{Checkpoint object}}
    \State{}\textbf{Class} \intervalalg{\checkpointindex}{\intervalmidpoint{}{}{}}{\level{}}
    \Indent{}
    \State{} $self.index = \checkpointindex; self.point = \intervalmidpoint{}{}{}; self.level = \level{}$
    \State{} $self.\binaastate{\checkpointindex}{\levelend}{l} =$ \binaainit{}%
    \label{algline:binaa}
    \EndIndent{}
    \LineComment{$\binaastatevalmsg{\checkpointindex}{\levelend}{\level{}}{r}{i}$ is a message with \binaryaa{} data $\binaastateval{\checkpointindex}{\levelend}{\level{}}$, round number $r$, and sender index $i$}
    \State{}\textbf{method} \clsmethod{Init}{v}$\to \binaastatevalmsg{\checkpointindex}{\levelend}{\level{}}{1}{i}$:
    \Indent{}
    \State{} $\binaastatevalmsg{\checkpointindex}{\levelend}{l}{1}{i}\gets self.\binaastate{\checkpointindex}{\levelend}{e}$.\clsmethod{Init}{v}\label{algline:binaa_init}
    % \EndIf{}
    \State{} \textbf{return } $\binaastatevalmsg{\checkpointindex}{\levelend}{l}{1}{i}$
    \EndIndent{}
    \State{}\textbf{method} \clsmethod{HandleMsg}{\binaastatevalmsg{\checkpointindex}{\levelend}{l}{r}{j}}$\to \binaastatevalmsg{\checkpointindex}{\levelend}{l}{r}{i}$:
    \Indent{}
    \State{} \textbf{return }$ self.\binaastate{\checkpointindex}{\levelend}{l}$.\clsmethod{HandleMsg}{\binaastateval{\checkpointindex}{\levelend}{l},r,j}
    \EndIndent{}
    \State{}\textbf{method} \clsmethod{StartRound}{r}$\to $ $\binaastatevalmsg{\checkpointindex}{\levelend}{l}{r}{i}$:
    \LineComment{Starts new round $r$}
    \Indent{}
    \State{} \textbf{return }$ self.\binaastate{\checkpointindex}{\levelend}{l}$.\clsmethod{StartRound}{r}
    \EndIndent{}
    % \adithya{Where is the API for $self.\binaastate{\checkpointindex}{\levelend}{l}$.\clsmethod{StartRound}{r} defined?}
    \State{}\textbf{method} \clsmethod{TermRound}{r}$\to $ bool:
    \Indent{}
    \LineComment{Returns true if round $r$ terminated}
    \State{} \textbf{return }$ self.\binaastate{\checkpointindex}{\levelend}{l}$.\clsmethod{TermRound}{r}
    \EndIndent{}
    \State{}\textbf{method} \clsmethod{TermWeight}{}$\to \binaastateweight{\checkpointindex}{\levelend}{l}$:
    \Indent{}
    \LineComment{Returns true if round $r$ terminated}
    \State{} \textbf{return }$ self.\binaastate{\checkpointindex}{\levelend}{l}$.\clsmethod{TermWeight}{}
    \EndIndent{}
  \end{algorithmic}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> Protocol/level.tex <==
\begin{algorithm}
  \small
  \caption{Level}
  \begin{algorithmic}[1]
    \Statex{} {\color{myorange}\(\triangleright\) \textrm{Level object}}
    \State{}\textbf{Class }\levelalg{l}{\overshoot{}}
    \Indent{}
    \State{} $self.level \leftarrow l;self.sep \leftarrow \overshoot{};self.checkpoints \leftarrow \{\}$;
    \EndIndent{}
    \LineComment{Returns a list of interval messages}
    \State{}\textbf{method} \clsmethod{Init}{\oracleinput{i}}$\to \levelmsgwrapper{\levelmsg}{i}$:
    \Indent{}
    \State{}Define \checkpointindices{} to be the set of all integers between $\frac{\levelstart}{self.sep},\frac{\levelend}{self.sep}$
    \State{}Define $\checkpointindex$th checkpoint as $\intervalmidpoint{\checkpointindex}{}{l} = \checkpointindex\times self.sep$
    \LineComment{Define Checkpoint objects}
    \For{$\checkpointindex \in \checkpointindices$}
    \State{} $\interval{\checkpointindex}{c+1}{l}\gets$\textbf{new }\intervalalg{\checkpointindex}{\checkpointindex{} \times self.sep{}}{l}
    \EndFor{}
    \State{} $\intervalmidpoint{\closestcc-1}{}{l},\intervalmidpoint{\closestcc}{c+1}{l}\gets$Two closest checkpoints to \oracleinput{i}
    \LineComment{Init with 1 to \interval{\closestcc-1}{\closestcc}{l},\interval{\closestcc}{\closestcc}{l} and 0 to others}
    \State{} \levelmsg$\gets\cup_{\checkpointindex\in\checkpointindices\setminus\{\closestcc-1,\closestcc\}}$ \interval{\checkpointindex}{c-1}{l}.\clsmethod{Init}{0}$\cup$\newline \tab\tab\tab\interval{\closestcc-1}{c+1}{l}.\clsmethod{Init}{1}$\cup$ \interval{\closestcc}{\levelend}{l}.\clsmethod{Init}{1}\label{algline:intervals_initiate}
    \State{} $self.checkpoints$.\clsmethod{Insert}{\interval{\checkpointindex}{c-1}{l}} $\forall \checkpointindex\in\checkpointindices$
    \State{} \textbf{return } $\levelmsgwrapper{\levelmsg}{i}$
    \EndIndent{}


    \State{}\textbf{method} \clsmethod{HandleMsg}{\levelmsg}$\to \levelmsgwrapper{\levelmsg}{l}$:
    \Indent{}
    \State{} \levelmsg$\gets\{\}$\Comment{List of messages to Broadcast}
    \For{$\binaastatevalmsg{\checkpointindex}{y}{\level{}}{r}{j}\in\levelmsg$}
    \State{} Fetch checkpoint \interval{\checkpointindex}{y}{l} from $self.checkpoints$
    \State{} \levelmsg$\gets \levelmsg \cup$ \interval{\checkpointindex}{y}{l}.\clsmethod{HandleMsg}{\binaastatevalmsg{x}{y}{l}{r}{j}}
    \EndFor{}
    \textbf{return } $\levelmsgwrapper{\levelmsg}{l}$
    \EndIndent{}


    \State{}\textbf{method } \clsmethod{StartRound}{r}$\to \levelmsgwrapper{\levelmsg}{i}$:
    \Indent{}
    \State{}\levelmsg$\gets\{\}$\Comment{List of messages to broadcast}
    \For{\interval{\checkpointindex}{y}{l}$\in self.checkpoints$}
    \State{}\levelmsg$\gets\levelmsg\cup$ \interval{\checkpointindex}{y}{l}.\clsmethod{StartRound}{r}
    \EndFor{}
    \textbf{return } $\levelmsgwrapper{\levelmsg}{i}$
    \EndIndent{}

    \State{}\textbf{method } \clsmethod{EndRound}{r}$\to$ bool:
    \Indent{}
    \State{} \textbf{return } true if all intervals in $self.checkpoints$ return true for $\interval{\checkpointindex}{y}{l}$.\clsmethod{TermRound}{r}
    \EndIndent{}
	\end{algorithmic}%
	\label{alg:level}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> Protocol/overview_fig.tex <==
\def\x{4}
\def\y{0.65}
\def\q{1}
\def\blk{\q+3*\y}
\def\blkt{4*\q+4*\y}
\def\blkth{\blkt+2*\q+4*\y}
\def\blkf{\blkth+2*\q+\y}
\begin{figure*}
	\begin{tikzpicture}
		\draw (0,3*\y) rectangle node{$\eaggrprot_{\round-2\frequency,1}$} ++(\q,\y);
		\draw (\q,3*\y) rectangle node{$\eaggrprot_{\round-\frequency,1}$} ++(\q,\y);
		
		
		\draw (0,2*\y) rectangle node{$\eaggrprot_{\round-2\frequency,2}$} ++(\q,\y);
		
		\draw (0,\y) rectangle node{$\eaggrprot_{\round-2\frequency,3}$} ++(\q,\y);
		\draw (\q,\y) rectangle node{$\eaggrprot_{\round-\frequency,3}$} ++(\q,\y);
		
		
		\draw (\q,0) rectangle node{$\eaggrprot_{\round-\frequency,4}$} ++(\q,\y);
		
		
		\draw (2*\q,4*\y) rectangle node {\rotatebox{270}{$\text{\bawss}(\batchsize+n)$}} ++(\y,-1*4*\y);
		\draw (2*\q+\y,4*\y) rectangle node{\rotatebox{270}{\gatherprot(\gatherset{i})}} ++(\y,-1*4*\y);
		\draw[->] (2*\q+2*\y,2*\y) -- (2*\q+3*\y,2*\y);
		
		
		\draw (\blk+\q,3*\y) rectangle node{$\eaggrprot_{\round-\frequency,1}$} ++(\q,\y);
		\draw (\blk+2*\q,3*\y) rectangle node{$\eaggrprot_{\round,1}$} ++(\q,\y);
		
		
		\draw (\blk+2*\q,2*\y) rectangle node{$\eaggrprot_{\round,2}$} ++(\q,\y);
		
		
		\draw (\blk+\q,\y) rectangle node{$\eaggrprot_{\round-\frequency,3}$} ++(\q,\y);
		\draw (\blk+2*\q,\y) rectangle node{$\eaggrprot_{\round,3}$} ++(\q,\y);
		
		
		\draw (\q+\blk,0) rectangle node{$\eaggrprot_{\round-\frequency,4}$} ++(\q,\y);
		\draw (\blk+2*\q,0) rectangle node{$\eaggrprot_{\round,4}$} ++(\q,\y);
		\draw[dashed,->] (4*\q+3*\y,2*\y) -- (4*\q+4*\y,2*\y);
		
		
		% BLOCK 2
		\draw (\blkt,3*\y) rectangle node{$\eaggrprot_{\round-\frequency,1}$} ++(\q,\y);
		\draw (\blkt+\q,3*\y) rectangle node{$\eaggrprot_{\round,1}$} ++(\q,\y);
		
		\draw (\blkt+\q,2*\y) rectangle node{$\eaggrprot_{\round,2}$} ++(\q,\y);
		
		
		\draw (\blkt,\y) rectangle node{$\eaggrprot_{\round-\frequency,3}$} ++(\q,\y);
		\draw (\blkt+\q,\y) rectangle node{$\eaggrprot_{\round,3}$} ++(\q,\y);
		
		\draw (\blkt,0) rectangle node{$\eaggrprot_{\round-\frequency,4}$} ++(\q,\y);
		\draw (\blkt+\q,0) rectangle node{$\eaggrprot_{\round,4}$} ++(\q,\y);
		
		
		\draw (\blkt+2*\q,4*\y) rectangle node {\rotatebox{270}{$\text{\bawss}(\batchsize)$}} ++(\y,-1*4*\y);
		\draw (\blkt+2*\q+\y,4*\y) rectangle node{\rotatebox{270}{\gatherprot(\gatherset{i})}} ++(\y,-1*4*\y);
		\draw (\blkt+2*\q+2*\y,4*\y) rectangle node{\rotatebox{270}{\commelectproc(\committee)}} ++(\y,-1*4*\y);
		\draw[->] (\blkt+2*\q+3*\y,2*\y) -- (\blkt+2*\q+4*\y,2*\y);
		\draw[dotted,->] (\blkt,3*\y) -- (\blkt-\y,-0.7*\y);
		\draw[dotted,->] (\blkt,\y) -- (\blkt-\y,-0.7*\y);
		\draw[dotted,->] (\blkt,0) -- (\blkt-\y,-0.7*\y);
		\node[circle,draw,scale=0.8] (c) at (\blkt-1.8*\y,-1.05*\y){\beacon{i}};
		
		\draw (\blkth,3*\y) rectangle node{$\eaggrprot_{\round,1}$} ++(\q,\y);
		
		
		\draw (\blkth,2*\y) rectangle node{$\eaggrprot_{\round,2}$} ++(\q,\y);
		\draw (\blkth+\q,2*\y) rectangle node{$\eaggrprot_{\round+\frequency,2}$} ++(\q,\y);
		
		\draw (\blkth,\y) rectangle node{$\eaggrprot_{\round,3}$} ++(\q,\y);
		\draw (\blkth+\q,\y) rectangle node{$\eaggrprot_{\round+\frequency,3}$} ++(\q,\y);
		
		
		\draw (\blkth,0) rectangle node{$\eaggrprot_{\round,4}$} ++(\q,\y);
		\draw (\blkth+\q,0) rectangle node{$\eaggrprot_{\round+\frequency,4}$} ++(\q,\y);
		\draw[dashed,->] (\blkth+2*\q,2*\y) -- (\blkth+2*\q+\y,2*\y);
		
		
		\draw (\blkf,3*\y) rectangle node{$\eaggrprot_{\round,1}$} ++(\q,\y);
		\draw (\blkf,2*\y) rectangle node{$\eaggrprot_{\round,2}$} ++(\q,\y);
		
		\draw (\blkf+\q,2*\y) rectangle node{$\eaggrprot_{\round+\frequency,2}$} ++(\q,\y);
		
		
		\draw (\blkf,\y) rectangle node{$\eaggrprot_{\round,3}$} ++(\q,\y);
		\draw (\blkf+\q,\y) rectangle node{$\eaggrprot_{\round+\frequency,3}$} ++(\q,\y);
		
		
		\draw (\blkf,0) rectangle node{$\eaggrprot_{\round,4}$} ++(\q,\y);
		\draw (\blkf+\q,0) rectangle node{$\eaggrprot_{\round+\frequency,4}$} ++(\q,\y);
		\draw (\blkf+2*\q,4*\y) rectangle node {\rotatebox{270}{$\text{\bawss}(\batchsize)$}} ++(\y,-1*4*\y);
		\draw (\blkf+2*\q+\y,4*\y) rectangle node{\rotatebox{270}{\gatherprot(\gatherset{i})}} ++(\y,-1*4*\y);
		\draw (\blkf+2*\q+2*\y,4*\y) rectangle node{\rotatebox{270}{\commelectproc(\committee)}} ++(\y,-1*4*\y);
		
		
		% Draw queue
		\node (b) at (0.1*\q,-1.05*\y) {\beaconqueue};
		\draw[-] (0.5*\y,-0.8*\y) -- (2*\q+0.5*\y,-0.8*\y);
		\draw[-] (0.5*\y,-1.3*\y) -- (2*\q+0.5*\y,-1.3*\y);
		\draw[-] (0.5*\y,-0.8*\y) -- (0.5*\y,-1.3*\y);
		\draw[-] (0.5*\q+0.5*\y,-0.8*\y) -- (0.5*\q+0.5*\y,-1.3*\y);
		%\draw[-] (0.75*\q,-0.8*\y) -- (0.75*\q,-1.3*\y);
		\draw[-] (\q+0.5*\y,-0.8*\y) -- (\q+0.5*\y,-1.3*\y);
		%\draw[-] (1.25*\q,-0.8*\y) -- (1.25*\q,-1.3*\y);
		\draw[-] (1.5*\q+0.5*\y,-0.8*\y) -- (1.5*\q+0.5*\y,-1.3*\y);
		%\draw[-] (1.75*\q,-0.8*\y) -- (1.75*\q,-1.3*\y);
		
		\node (b) at (0.1*\q,-1.05*\y-\y) {$\beaconqueue_c$};
		\draw[-] (0.5*\y,-0.8*\y-\y) -- (2*\q+0.5*\y,-0.8*\y-\y);
		\draw[-] (0.5*\y,-1.3*\y-\y) -- (2*\q+0.5*\y,-1.3*\y-\y);
		\draw[-] (0.5*\y,-0.8*\y-\y) -- (0.5*\y,-1.3*\y-\y);
		\draw[-] (0.5*\q+0.5*\y,-0.8*\y-\y) -- (0.5*\q+0.5*\y,-1.3*\y-\y);
		%\draw[-] (0.75*\q,-0.8*\y) -- (0.75*\q,-1.3*\y);
		\draw[-] (\q+0.5*\y,-0.8*\y-\y) -- (\q+0.5*\y,-1.3*\y-\y);
		%\draw[-] (1.25*\q,-0.8*\y) -- (1.25*\q,-1.3*\y);
		\draw[-] (1.5*\q+0.5*\y,-0.8*\y-\y) -- (1.5*\q+0.5*\y,-1.3*\y-\y);
		
		\draw[->] (c) -- node[above] {Add \batchsize beacons} (2*\q+0.5*\y,-1.05*\y);
		\draw[dotted,->] (\blkf,3*\y) .. controls (\blkf,-\y) .. (c);
		\draw[dotted,->] (\blkf,2*\y) .. controls (\blkf,-\y) .. (c);
		\draw[dotted,->] (\blkf,\y) .. controls (\blkf,-\y) .. (c);
		\draw[dotted,->] (\blkf,0) .. controls (\blkf,-\y) .. (c);
		
		\draw[dotted,->] (\blkf,3*\y) -- (\blkf-1*\y,-1.8*\y);
		\draw[dotted,->] (\blkf,2*\y) -- (\blkf-1*\y,-1.8*\y);
		\draw[dotted,->] (\blkf,\y) -- (\blkf-1*\y,-1.8*\y);
		\draw[dotted,->] (\blkf,0) -- (\blkf-1*\y,-1.8*\y);
		\node[circle,draw,scale=0.8] (com) at (\blkf-1.8*\y,-2.05*\y){\beacon{i}};
		\draw[->] (com) -- node[above] {Add $n$ beacons} (\blkth-1.5*\q,-2.05*\y) -- node[above] {} (2*\q+0.5*\y,-2.05*\y);
		
		\draw[dashdotted,->] (2*\q+0.5*\y,-2.05*\y) .. controls (\blkth-\q,-2.05*\y) .. (\blkth-\q,0);
		\draw[dashdotted,->] (com) -- node[above,align=center] {Invoke beacon from $\beaconqueue_c$} (\blkf+1.8*\q+2*\y,-2.05*\y) .. controls (\blkf+2*\q+2*\y,-2.05*\y) .. (\blkf+2*\q+2.5*\y,0);
		
		
		% Line above
		\draw[|-|] (0,4.5*\y) -- node[above] {Round $r=\frequency n$} (2*\q+2*\y,4.5*\y);
		\draw[|-|] (\blk+1.5*\y,4.5*\y) -- node[above] {Round $r+1$} (\blk+2*\q+1.5*\y,4.5*\y);
		\draw[|-|] (\blkt,4.5*\y) -- node[above] {Round $r+\frequency$} (\blkt+2*\q+3*\y,4.5*\y);
		\draw[|-|] (\blkth,4.5*\y) -- node[above] {Round $r+\frequency+1$} (\blkth+2*\q,4.5*\y);
		\draw[|-|] (\blkf,4.5*\y) -- node[above] {Round $r+2\frequency$} (\blkf+2*\q+3*\y,4.5*\y);
	\end{tikzpicture}
	\caption{\textbf{\protocol pipeline}: We describe the pipeline of \protocol with batch size \batchsize period $\frequency=\frac{\aatermrounds}{2}$. \protocol initiates a new \bawss instance once every \frequency rounds and pipelines the corresponding \approxconsensus instances $\eaggrprot_{\round,i}$. \protocol also initiates preparation of $n$ more  beacons once every $\frequency n$ rounds. These beacons are prepared without committee election, and therefore run $\eaggrprot_{\round,j}$ for all $n$ nodes. \protocol moves to the next round only after terminating \bawss,\gatherprot, and round $\round$ of $\eaggrprot_{.}$ instances in the pipeline. After completing $\aatermrounds=2\frequency$ rounds, \batchsize beacons initiated before \aatermrounds rounds are added to \beaconqueue to be eventually reconstructed. Further, the extra $n$ beacons prepared in round $\round$ are added into a separate queue $\beaconqueue_c$, used for electing committees for future beacons in rounds $\round: \round\mod\frequency=0, \round\mod n \neq 0$.}
	\label{fig:pipeline_overview}
\end{figure*}

==> Protocol/rz_protocol.tex <==
\begin{algorithm}
	\label{alg:rz}
	\caption{\protocolaa: Protocol for \approxconsensus}
	\begin{algorithmic}[1]
		\State \textbf{INPUT}: \initialvalue{i}\Comment{Sampled from distribution f(x)}
		\State Public parameters: \pk{j} for j $\in$ \noderange{1}{n}
		\State \textbf{OUTPUT}: $V$
		\HorizontalLine
		\LineComment{Run \protocolapd with input \hmessage{i}=\initialvalue{i}} 
		\State \valueset{i} := \protocolapd(\initialvalue{i})\Comment{Exchange values using \protocolapd in \cref{alg:apd}}
		\LineComment{Reduce \valueset{i} as in~\cite{abraham2004approxagreement}}
		\State $\valueset{i} \leftarrow \trim{\sort{\valueset{i}}}{\faults}$ \Comment{The function $\trim{\valueset{i}}{\faults}$ trims out $\faults$ values from each end of the set \valueset{i} \cite{abraham2004approxagreement}}
		\State $\initialvalue{i} \leftarrow \frac{\minimum{\valueset{i}} + \maximum{\valueset{i}}}{2}$ \Comment{Average the extremes}
		\LineComment{Run the \protocoloaa~\cite{abraham2004approxagreement} with updated \initialvalue{i}}
		\State \textbf{OUTPUT}: \protocoloaa(\initialvalue{i})
	\end{algorithmic}
\end{algorithm}

==> Protocol/threshold_enc.tex <==
 \textbf{Probabilistic analysis}: The total number of ways in which a $CS$ can be chosen by the adversary with $n-2f$ honest values is equivalent to the number of ways in which we can select $n-2f$ nodes from $n-f$ honest nodes. Given that the ground truth variable $X = 1$ and every honest node measures $X$ correctly with a probability of $p$, the probability with which the convergence can be forced to $0$ can be calculated using random variable math. Let $R$ denote the random variable governing the output of the $RZ$-protocol. As specified previously, the IND-CPA security of the threshold encryption scheme ensures that the adversary has to choose $n-2f$ values from $n-f$ honest nodes' values in a randomized fashion. In the setting described in $\cref{fig:oligarchy_flow}$, let the honest nodes $N1,N3,N4$ measure values $\{0,1,1\}$. The sets $\{0,1\},\{0,1\},\{1,1\}$ are all equally likely to be part of the ACS, $\implies P[\{0,1\} \in CS] = \frac{1}{3}, P[\{1,1\} \in CS] = \frac{2}{3}$. We divide the analysis into two parts: 
\begin{enumerate}
    \item The adversary gets $\{0,1\}$ to be part of the CS. In this case, the consensus converges to $0$ with probability $2/3$. 
    \item The adversary gets $\{1,1\}$ to be part of the CS.  The output of the first round is as follows. The set of messages received by each node is denoted as $\{m_{1},m_2,m_3,m_4\}$. $x$ denotes that the node did not receive a message in that slot.  
    \begin{enumerate}
        \item $N1 - \{0,1,1,0\}$
        \item $N3 - \{x,1,1,0\}$
        \item $N4 - \{x,1,1,0\}$
    \end{enumerate}
    After elimination and mean reduction, $N1 = 0.5$, $N3 = 1$ and $N4=1$. From round 2, the adversary has full power to dictate convergence from round 2 because value privacy is not in effect anymore. Hence, the convergence happens at $R=0.5$ with probability $\frac{2}{3}$.   
\end{enumerate}

==> Protocol/wtprotocol.tex <==
\subsection{Witness Technique}
The witness technique was proposed by Abraham et al. in \cite{abraham2004approxagreement}. The technique was employed in the protocol proposed to achieve \approxconsensus. We denote this protocol by the acronym \protocol{WT}. We briefly describe the protocol in this section. We assume a set of nodes \noderange{1}{n}, each possesses a value \initialvalue{i}. The honest nodes wish to come to \approxconsensus, with a predetermined $\epsilon$. We also assume that the protocol must tolerate \faults = \floor{\frac{n}{3}} faults $\implies n = 3\faults + 1$. The protocol described in \cite{abraham2004approxagreement} is written in \cref{alg:witness_technique}. When every node reliably broadcasts its initial value \initialvalue{i}, an honest node can only wait for \highthreshold messages because of the asynchronous network setting. Every honest node that receives \highthreshold messages will have \faults+1 messages in common with every other honest node that has received \highthreshold messages. The number of messages in common between two honest nodes can be increased to \highthreshold with the help of the witness technique. Instead of waiting to accept \highthreshold messages, every honest node waits until accepting \highthreshold witnesses. 

\paragraph{Witness}: An honest node $j$ is a witness to another honest node $i$ if $i$ has accepted the first \highthreshold messages that $j$ has accepted. The set of witnesses to node $i$ is updated as follows.
\begin{equation}
	(\reportset{i}{j}\cap \valueset{i} \ge \highthreshold) \implies (\witnesses{i} = \witnesses{i} \cup j)
\end{equation}
The list of first \highthreshold messages received by node $j$ is stored in the variable \reportset{i}{j} by node $i$. The set of values received by node $i$ is stored in the variable \valueset{i}. The set of witnesses for node $i$ is stored in the variable \witnesses{i}. 

Every honest node moves to round $r+1$ only after receiving \highthreshold witnesses in round $r$. Every pair of honest nodes has at least \minthreshold witnesses in common, out of which at least one witness is honest. Hence, every pair of honest nodes has at least one honest witness in common, which implies that they accepted at least \highthreshold messages in common. 

After receiving \highthreshold witnesses, an honest node applies the reduce procedure \reduce{i}{\valueset{i}} on the value set \valueset{i}. The \textit{Reduce} procedure is described in \cref{alg:reduce_proc}. After each round, the range of honest nodes' values reduces by a factor of $\frac{1}{2}$. The honest nodes also run a round estimation protocol prior to \cref{alg:witness_technique} to estimate the range of honest nodes' initial values. According to this estimate, the honest nodes run \protocol{WT} for $r$ rounds. The round estimation protocol is described in \cref{alg:round_estimation}.  
\begin{algorithm}
\caption{\protocol{WT} \cite{abraham2004approxagreement}}\label{alg:witness_technique}
As honest node $i$ participating in the protocol.\\
\textbf{Input}: \initialvalue{i}\\
% No. of rounds to run is important to know
// Estimate the number of rounds to execute\\
\initialvalue{i},\rounds $\leftarrow$ \estimaterounds{i}{\initialvalue{i}}\\
% temporary variable for keeping track of how many rounds have been run
$r_t \leftarrow 1$;\\
\While{$r_t \le r$}{
\rbroadcast{i}{\initialvalue{i}}\\
% got n-t witnesses?
$\valueset{i} \leftarrow \{\}; \reports{i} \leftarrow \{\}; \reportset{i}{j} \leftarrow \{\} \forall j \in \noderange{1}{n}; \witnesses{i} \leftarrow \{\}$\\
\While{$|\witnesses{i}| \le \highthreshold$}{
    On reliably accepting \initialvalue{j}:\\
    	\tab // Add value to ValueSet
        \tab $\valueset{i} \leftarrow \valueset{i} \cup \initialvalue{j}$\\
        \tab // Send report to every node
        \tab $\report{i}{j} \leftarrow \langle \initialvalue{j},\sign{i}{\initialvalue{j}} \rangle$\\
        \tab // Add report to reports set\\
        \tab $\reports{i} \leftarrow \reports{i} \cup \report{i}{j}$\\
    // Wait until receiving \highthreshold messages\\
	On $|\reports{i}| \ge \highthreshold$:\\
		\tab // Send ReportSet to every node\\
		\tab \sendall{i}{\reports{i}}\\
    On accepting \reports{j} and verifying signatures:\\
    	\tab // Add report to ReportSet
        \tab $\reportset{i}{j} \leftarrow \reports{j}$\\
        \tab \If{$|\reportset{i}{j}\cap \valueset{i}| \ge \highthreshold$}{
            \tab $\witnesses{i} \leftarrow \witnesses{i} \cup j$\\
        }
}
$\initialvalue{i} \leftarrow \reduce{\valueset{i}}{\faults}$\\
$r_t \leftarrow r_t + 1$\\
}
\textbf{Output}: \initialvalue{i}
\end{algorithm}

% Round estimation algorithm
\begin{algorithm}
    \caption{Round estimation protocol \cite{abraham2004approxagreement}}
    \label{alg:round_estimation}
    \textbf{Input}: \initialvalue{i},$\epsilon$\\
\rbroadcast{i}{\initialvalue{i}}\\
$\valueset{i} \leftarrow \{\}; \reportset{i}{j} \leftarrow \{\} \forall j \in \noderange{1}{n}; \witnesses{i} \leftarrow \{\}$\\
\While{$|\witnesses{i}| \le \highthreshold$}{
    On reliably accepting \initialvalue{j}:\\
    	// Create a report message\\
        \tab $\report{i}{j} \leftarrow \langle \initialvalue{j},\sign{i}{\initialvalue{j}} \rangle$\\
        \tab // Add reports to report set\\
        \tab \reports{i} $\leftarrow$ \reports{i} $\cup$ \report{i}{j}\\
    On $|\reports{i}| \ge \highthreshold$:\\
    	\tab // Reliably broadcast ReportSet\\
  		\tab \rbroadcast{i}{\reports{i}}\\
    On reliably accepting \reports{j} and verifying signatures:\\
    	\tab // Add all reports to ReportSet\\
        \tab $\reportset{i}{j} \leftarrow \reports{j}$\\
        \tab \If{$|\reportset{i}{j}\cap \valueset{i}| \ge \highthreshold$}{
            \tab $\witnesses{i} \leftarrow \witnesses{i} \cup j$\\
        }
    }
\For{$k \in \witnesses{i}$}{
    $\valueset{i} \leftarrow \valueset{i} \cup \reduce{\reportset{i}{k}}{\faults}$\\
}\label{algstep:update_vi}
$\initialvalue{i} \leftarrow \reduce{\valueset{i}}{\faults}$\\
$\textit{rounds} \leftarrow \log_{2}(\frac{\range{\valueset{i}}}{\epsilon})$\\
\textbf{Output}: \initialvalue{i},\textit{rounds}
\end{algorithm}

% Reduce algorithm
\begin{algorithm}
    \caption{\reduce{S}{\faults} - Set reduction function \cite{abraham2004approxagreement}}\label{alg:reduce_proc}
    \textbf{Input}: S,\faults\\
    The function $\trim{S}{\faults}$ trims out $\faults$ values from each end of the set $S$. \\
    $S \leftarrow \trim{\sort{S}}{\faults}$\\
    $\textit{out} \leftarrow \frac{\minimum{S} + \maximum{S}}{2}$\\
    \textbf{Output}: \textit{out}
\end{algorithm}

%Commented out
\iffalse
\rebox
	\begin{figure}[!tbp]
		\caption{The witness technique protocol or \protocol{WT} described by Abraham et al. in \cite{abraham2004approxagreement}}
		\label{protocol:wt}
		\begin{flushleft}
			We describe the protocol presented by Abraham et al. in \cite{abraham2004approxagreement}. Nodes \noderange{1}{n} participate in the protocol with initial values \initialvalue{i} $\forall i \in \noderange{1}{n}$. We assume that the total number of faults is \faults.  The protocol is divided into two different phases. 
			\begin{enumerate}
				\item An honest node $i$ reliably broadcasts its value. 
				\begin{equation}
					\rbroadcast{i}{\initialvalue{i}}
				\end{equation}
				\item When an honest node $i$ reliably delivers a value from node $j$ by invoking \rdeliver{i}{\initialvalue{j}}, it constructs a report message $\report{i}{j} = \langle \initialvalue{j},\sign{i}{\initialvalue{j}}\rangle$. It reliably broadcasts the report by invoking \sendall{i}{\report{i}{j}}. 
				\item An honest node $i$ collects the first \highthreshold report messages from every other honest node $j$ into \reportset{i}{j}. 
				\item \paragraph{Witness} If an honest node $i$'s value set \valueset{i} has at least \highthreshold number of messages in common with a report set \reportset{i}{j} of another honest node $j$, then honest node $j$ is a witness for node $i$. Every honest node $i$ maintains a set of witnesses \witnesses{i} and adds node $j$ to the witness once the condition is satisfied. 
				\begin{equation}
					(\valueset{i}\cup \reportset{i}{j}) \Rightarrow (\witnesses{i} = \witnesses{i} \cup j)
				\end{equation}
				\item An honest node $i$ waits until collecting \highthreshold witnesses. It updates the value for its next round by reducing its value set \valueset{i}. 
				\begin{equation}
					\initialvalue{i} = \textit{reduce}(\valueset{i})
				\end{equation}
			\end{enumerate}
		\end{flushleft}
	\end{figure}
	\unbox
	\fi

==> bin_aa.tex <==
\subsection{Binary Approximate Agreement}
Next, we address the inefficiencies in prior \approxconsensus protocols like \abrahamapprox~\cite{abraham2004approxagreement} and \bundledaa~\cite{freitas2022distributed}. The \approxconsensus phase of \protocol controls the degree of agreement amongst honest nodes. As described in ~\cref{fig:working_coin}, the probability of agreement $\delta$ depends on the proximity of the outputs. For a fault-tolerance of $n=3f+1$, the SOTA \approxconsensus protocol is Abraham \etal's protocol~\cite{abraham2004approxagreement}. However, n-parallel instances of Abraham \etal's protocol cost \bigo{n^4} complexity. Hence, Freitas \etal~\cite{freitas2022distributed} proposed a new primitive called Bundled Approximate Agreement(\bundledaa), where nodes use a single reliable broadcast to disseminate messages concerning all $n$ \approxconsensus instances. Every \bundledaa iteration involves an $n$-parallel reliable broadcast and 4 rounds to complete, which is expensive. For example, achieving $\delta = 1-10^{-12}$ for an $n=10$ node system would require 210 rounds, run erasure encoding and decoding(or error correction codes based on the type of RBC) 126 times, and send ~21000 messages. Although the communication complexity is \bigo{\kappa n^3 \log(n)}, the hidden constants for \bundledaa are high, which results in an inefficient protocol.

We observe that the n-parallel RBC and the witness technique comprising \fktprotocol's \bundledaa primitive are only required when the inputs of honest nodes are multivalent and unconstrained. Multiple protocols in the literature introduced some level of constraints on honest nodes' inputs to improve the cost incurred by n-parallel RBC. For example, the Validated Asynchronous Byzantine Agreement (VABA)~\cite{abraham2019asymptotically} introduced by Abraham \etal and Multi-Valued Validated Byzantine Agreement (MVBA) introduced by Cachin \etal~\cite{cachin2001secure} assume an external validity function $f(x)$ available to all honest nodes to verify the Validity of the input. This constraint on honest inputs and output enabled the development of efficient protocols with comm. complexity \bigo{\kappa n^2} without using $n$-parallel RBC. Similar to such protocols, we introduce an \approxconsensus protocol by constraining the inputs to be binary. 

%\input{Protocol/binary_appx_consensus}

When the inputs are binary within $\{0,1\}$, the $n$-parallel RBC in each round of \approxconsensus can be replaced with a cheaper primitive called Crusader agreement~\cite{abraham2022efficient}, a constituent part of Binary BA protocols. Crusader agreement mandates that nodes in a bivalent initial state $\{0,1\}$ must move to a state with weaker agreement where nodes can output \bottom, but not two different values. We describe the Binary Approximate Agreement protocol(\binaryaa) in ~\cref{alg:bin_appx_consensus}. Each node starts with values $c_0$ and $c_1$ ($0$ and $1$ in \protocol), both of which need to be publicly known. Each node sends an $ECHO$ message for its value. It also amplifies another value by sending an $ECHO$ if it received $t+1$ such $ECHO$s for the value. We note that values possessed by only malicious nodes can never receive $t+1$ $ECHO$ messages. Once it receives $2t+1$ $ECHO$ messages for a value, it broadcasts an $ECHO2$ message. It waits until it receives $2t+1$ $ECHO$s for two different values to output \bottom or 2t+1 $ECHO2$ messages for a single value to output the value. Starting a bivalent state in round 1, if a node outputs \bottom in round one, it updates its value to $\frac{0+1}{2} = 0.5$ and moves to the next round. Therefore, the state of honest nodes in round 2 is also bivalent, but with the range reduced by $\frac{1}{2}$.

This primitive is inexpensive with \bigo{n^2} complexity per round, takes two round trips to complete, and does not use any message encoding. After running for $\log(\frac{1}{\aaprecision})$ rounds, the nodes achieve \approxconsensus and remain in a bivalent state. This protocol has a communication complexity of \bigo{n^2\log^2(1/\aaprecision)}, with each message of size $\log(1/\aaprecision)$. \protocol requires $n$ instances of BinAA to run in parallel, which results in a comm. complexity of \bigo{n^3\log^2(1/\aaprecision)}.

\paragraph{Reducing message complexity} Other asynchronous BFT protocols like Speeding Dumbo~\cite{guo2022speedingdumbo} and Narwhal~\cite{george2022narwhal} emphasize the importance of low message complexity in protocol efficiency and aim to minimize message complexity in the optimistic case. $n$ instances of \binaryaa have a message complexity of \bigo{n^3} because of $n$ all-to-all broadcasts. To reduce this, our implementation of \binaryaa in \protocol shares broadcasts over all n \binaryaa instances. We batch $ECHO$ and $ECHO2$ messages of all $n$ \binaryaa instances to reduce message complexity. Except in cases of amplification where a node cannot wait to bunch messages, every node waits until having $ECHO$ and $ECHO2$ messages for all $n$ instances. Without active adversarial scheduling, this batching technique has an optimistic message complexity of \bigo{n^2} and a worst-case complexity of \bigo{n^3}. With this optimization, the approximate agreement phase in \protocol in an $n=4$ system and $\delta = 1-10^{-12}$ takes 84 round trips, no message encoding, and $~$2000 messages to terminate.

We present the proofs of Termination, \approxconsensus, and Validity. 
\begin{lemma}
	The protocol described in ~\cref{alg:bin_appx_consensus} satisfies termination property of \approxconsensus primitive.
\end{lemma}
\begin{proof}
	We show that the protocol must terminate a started round $r<=r_t$. Given that there are at least $2t+1$ honest nodes where each node has one of two values $c_0$ or $c_1$, there must be at least one value $c_0$ or $c_1$ that is possessed by $t+1$ honest nodes. At least one value must receive $2t+1$ $ECHO$ messages, which implies every honest node must broadcast an $ECHO2$ message. We show that if an honest node does not receive $2t+1$ $ECHO2$ messages, it must receive $2t+1$ ECHO messages for both values. Given that node $i$ is set up never to receive $2t+1$ $ECHO2$ messages, which implies that $i$ must receive two different $ECHO2$ messages for both $c_0$ and $c_1$ from honest nodes. Since at least one honest node each sent $ECHO2$s to $i$ for $c_0$ and $c_1$, they must have received $2t+1$ $ECHOs$ for $c_0$ and $c_1$. As $c_0$ and $c_1$ both have $2t+1$ $ECHO$s, $i$ will eventually receive $2t+1$ $ECHO$s for both $c_0$ and $c_1$. Therefore, the protocol must terminate round $r$. There is a global agreement on $c_0$ and $c_1$, so the protocol strictly runs for $r_t$ rounds.
\end{proof}
\begin{lemma}
	The protocol described in ~\cref{alg:bin_appx_consensus} satisfies \approxconsensus property of \approxconsensus primitive.
\end{lemma}
\begin{proof}
	We first prove that if the protocol is in a bivalent state in round $r$, it must move to a bivalent or univalent state in round $r+1$. Assuming nodes start round $r$ of the protocol with values $c_0'$ and $c_1'$. From the properties of Crusader agreement, the protocol moves into state $\{c_0',\bottom\}$ or ${c_1',\bottom}$. Honest nodes receiving \bottom update their value to $v = \frac{c_0'+c_1'}{2}$, which implies that the range of honest values reduces to $\frac{c_1'-c_0'}{2}$. 
	
	In contrast, if the state after round $r$ is univalent, the nodes have already agreed, which implies that the range of honest inputs reduces by at least a factor of $\frac{1}{2}$. Therefore, after at most $\log_2(\frac{1}{\aaprecision})$ rounds, the protocol achieves \approxconsensus. 
\end{proof}
\begin{lemma}
	The protocol described in ~\cref{alg:bin_appx_consensus} satisfies Validity property of \approxconsensus primitive.
\end{lemma}
\begin{proof}
	We observe that the updated value in each round must receive $2t+1$ $ECHO$ messages. Every value part of the set $T_i$ must have at least $t+1$ nodes send $ECHO$ messages. Any value not possessed by honest nodes at the start cannot receive $t+1$ $ECHO$s, and therefore, a value outside the range of $c_0,c_1$ cannot be added to the set $T_i$. Since averaging is the only operation on the values in $T_i$, the output decision must lie within the range of initial inputs. Similarly, if nodes start the protocol from a univalent state, no other value will get $t+1$ $ECHO$s, and the nodes will decide on the starting value, satisfying Validity.
\end{proof}

Overall, the amortized communication complexity per coin creation of \protocol is \bigo{\kappa n^2\log(n)+ n^2\log^2(n/(1-\delta))}, an \bigo{n} factor of improvement over \fktprotocol. The reconstruction phase of \protocol costs \bigo{n^3\log(n)} with an \bigo{n^2} message complexity. 

==> symbol-table.tex <==
\begin{table}
	\centering
	\newcolumntype{s}{>{\centering\hsize=.3\hsize}X}
	\newcolumntype{Y}{>{\centering\arraybackslash}X}
	\caption{Symbols and notations used in \protocol}
	\begin{tabularx}{\linewidth}[!ht]{s Y}
		\hline\hline
		Symbol & Description \\
		\hline\hline
		\statparam & Statistical security parameter\\
		\secparam & Computational security parameter\\
		\batchsize & Batch size in \bawss \\
		\frequency & Period of \bawss \\
		\domain & Range of beacons \\
		\round & Current round of \protocol \\
		\bawss$_{\round,i}$ & \bawss instantiated by node \node{i} in round \round of \protocol\\
		\secrets{\round,i} & The set of \batchsize secrets shared by \node{i} through round \round's \bawss instance\\
		$\committee_{\round}$ & The committee elected for \bawss$_{\round,.}$\\
		\gatherset{\round,i} & The output from \gatherterm{\round,i} for a \bawss$_{\round,.}$ \\
		$\eaggrprot_{\round,i}$ & \approxconsensus instance corresponding to \bawss$_{\round,i}$ instantiated in \protocol round \round\\
		\beaconqueue & The list of all prepared beacons yet to be opened\\
		$\beaconqueue_c$ & The list of all prepared beacons for committee election\\
		\hline
	\end{tabularx}
\end{table}

==> tables/exhaustive-related-work.tex <==
\begin{table*}
	\footnotesize
	\renewcommand{\thefootnote}{\fnsymbol{footnote}}
	%\def\footnoteLeaderOnly{\footnotemark[4]}
	\def\footnoteCC{\footnotemark[2]}
	\def\footnoteValidity{\footnotemark[4]}
	\def\footnoteDelphiBID{\footnotemark[5]}
	\def\footnoteAppxAggr{\footnotemark[6]}
	\def\footnoteDora{\footnotemark[1]}
	\def\footnoteFin{\footnotemark[3]}
	%\def\footnoteMulWithoutThresh{\footnotemark[5]}
	%\def\footnoteProvBroadcast{\footnotemark[6]}
	%\def\footnoteNarwhalThresh{\footnotemark[7]}
	%\small
	\centering
	\caption[Related work comparison]{\small Comparison of relevant Asynchronous BA protocols
	}%
	\label{tab:relwork_combined}
	\newcolumntype{s}{>{\centering\hsize=.25\hsize}X}
	\newcolumntype{Y}{>{\centering\arraybackslash}X}
	\newcolumntype{Z}{>{\hsize=1.4\hsize}X}
	\newcolumntype{d}{>{\centering\hsize=.6\hsize}X}
	\newcolumntype{k}{>{\centering\hsize=.6\hsize}X}
	\newcolumntype{M}{>{\centering\arraybackslash\hsize=1.8\hsize}X}
	\centering
	\begin{tabularx}{\linewidth}[!ht]{Z M Y d d d Y Y}
		\toprule
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Protocol}\endtabular}
		&
		%\rotatebox{90}{\tabular{@{}l@{}}\textbf{Network}\endtabular}
		%&
		%\rotatebox{90}{\tabular{@{}l@{}}\textbf{Fault}\\ \textbf{Tolerance}\endtabular}
		%&
		%&
		%\rotatebox{90}{\tabular{@{}l@{}}\textbf{Termination}\endtabular}
		%&
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Communication}\\ \textbf{Complexity}\endtabular} 
		&
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Message}\\ \textbf{Complexity}\endtabular}
		&
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Round}\\ \textbf{Complexity}\endtabular}
		&
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Signing}\\ \textbf{Complexity}\endtabular}
		&
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Verification}\\ \textbf{Complexity}\endtabular}
		%&
		%\rotatebox{90}{\tabular{@{}l@{}}\textbf{SMR Verification}\\ \textbf{Complexity}\endtabular}
		&
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Validity}\endtabular}
		&
		%\rotatebox{90}{\tabular{@{}l@{}}\textbf{Input }\\ \textbf{Assumption}\endtabular}
		%&
		\rotatebox{90}{\tabular{@{}l@{}}\textbf{Setup }\\ \textbf{Assumption}\endtabular}
		\\
		\midrule
		%Chainlink~\cite{breidenbach2021chainlink}
		%&
		%p sync.
		%&
		%1/3
		%&
		%D
		%&
		%\bigo{\sizeof{V}n^3 + \secparam n^4}
		%&
		%\bigo{n^3}
		%&
		%\bigo{n}
		%&
		%\bigo{n}
		%&
		%\bigo{n^3}
		%&
		%$[m,M]$
		%&
		%None
		%&
		%PKI
		%\\
		%DORA~\cite{kate2023dora}
		%&
		%async.
		%&
		%1/2
		%&
		%\bigo{n}
		%&
		%\bigo{n}
		%&
		%\bigo{1}
		%&
		%\bigo{1}
		%&
		%\bigo{n}
		%&
		%$[m-\maxrange,M+\maxrange]$
		%&
		%$\honestrange\leq\maxrange$
		%&
		%SMR channel
		%\\
		%DORA~\cite{kate2023dora}\footnoteDora
		%&
		%async.
		%&
		%1/3
		%&
		%D
		%&
		%\bigo{|V|n^3+\secparam n^3}
		%&
		%\bigo{n^2}
		%&
		%\bigo{1}
		%&
		%\bigo{n}
		%&
		%\bigo{n^2}
		%&
		%$[m,M]$
		%&
		%None
		%&
		%PKI
		%\\
		HoneyBadgerBFT~\cite{miller2016honey}
		%&
		%async.
		%&
		%1/3
		%&
		%R
		&
		\bigo{|V|n^2 + \secparam{} n^3}
		&
		\bigo{n^3}
		&
		\bigo{\log(n)}
		&
		\bigo{n}
		&
		\bigo{n^2}
		&
		$[m,M]$
		%&
		%None
		&
		DKG
		\\
		Dumbo2~\cite{guo2020dumbo}
		%&
		%async.
		%&
		%1/3
		%&
		%R
		&
		\bigo{|V|n^2+\secparam{} n^3}
		&
		\bigo{n^3}
		&
		\bigo{1}
		&
		\bigo{n}
		&
		\bigo{n^2}
		&
		$[m,M]$
		%&
		%None
		&
		HT-DKG
		\\
		Speeding Dumbo~\cite{guo2022speedingdumbo}
		%&
		%async.
		%&
		%1/3
		%&
		%R
		&
		\bigo{|V|n^2+\secparam{} n^3}
		&
		\bigo{n^2}
		&
		\bigo{1}
		&
		\bigo{n}
		&
		\bigo{n^2}
		&
		$[m,M]$
		%&
		%None
		&
		HT-DKG
		\\
		FIN~\cite{duan2023sigfreeacs}
		%&
		%async.
		%&
		%1/3
		%&
		%R
		&
		\bigo{|V|n^2+\secparam{} n^3}
		&
		\bigo{n^3}
		&
		\bigo{1}
		&
		\bigo{\log(n)}
		&
		\bigo{n\log(n)}\footnoteFin{}
		&
		$[m,M]$
		%&
		%None
		&
		DKG
		\\
		Abraham \etal~\cite{abraham2004approxagreement}\footnoteAppxAggr{}
		%&
		%async.
		%&
		%1/3
		%&
		%D
		&
		\bigo{|V|n^3\log(\frac{\honestrange}{\epsilon})+n^4}
		&
		\bigo{n^3\log(\frac{\honestrange}{\epsilon})}
		&
		\bigo{\log(\frac{\honestrange}{\epsilon})}
		&
		0
		&
		0
		&
		$[m,M]$
		%&
		%None
		&
		Auth.\ channels
		\\
		\midrule
		\protocol\footnoteDelphiBID\footnoteAppxAggr{}
		%&
		%async.
		%&
		%1/3
		%&
		%D
		&
		\bigo{|V|n^2\log(\frac{n\maxrange}{\epsilon})}
		&
		\bigo{n^2\log(\frac{n\maxrange}{\epsilon})}
		&
		\bigo{\log(\frac{n\maxrange}{\epsilon})}
		&
		0
		&
		0
		%&
		%\bigo{1}
		&
		$[m-\honestrange,M+\honestrange]$
		%&
		%$\honestrange\leq \maxrange$
		&
		Auth.\ channels
		\\
		\protocolrbc\footnoteAppxAggr{}
		%&
		%async.
		%&
		%1/3
		%&
		%D
		&
		\bigo{|V|n^2\log(\frac{n\honestrange}{\epsilon})+n^3}
		&
		\bigo{n^3}
		&
		\bigo{\log(\frac{n\honestrange}{\epsilon})}
		&
		0
		&
		0
		%&
		%\bigo{1}
		&
		$[m-\honestrange,M+\honestrange]$
		%&
		%None
		&
		Auth.\ channels
		\\
		\bottomrule
	\end{tabularx}
	\begin{flushleft}
		{\small 
			%\textbf{SMR Verification}: The number of signatures the SMR channel verifies to consume the output from oracles. 
			%In all protocols, oracles produce an attested output and submit it to the blockchain for consumption by smart contracts\cite[Section 5.4]{breidenbach2021chainlink}. This step is common for all protocols, so we do not count its cost in this table. 
			\footnoteDelphiBID{} \protocol{} (Bounded Input Difference) assumes an upper bound \maxrange{} on the difference between honest inputs \honestrange. \honestset{} is the set of all honest inputs, $m = \min(\honestset), M=\max(\honestset)$, $\honestrange = M-m$, and $\honestrange \leq \maxrange$.
			\textbf{Validity}: The protocol's output \oracleoutput{} is guaranteed to be within this range.\ \footnoteAppxAggr{} These protocols are Approximate Agreement protocols and achieve \approxconsensus{} with the specified Validity condition.
			\footnoteFin{} FIN uses a proposal election procedure, which requires a $n$-ary common coin which provides $\log(n)$ bits of distributed randomness. With a local PRNG, this complexity can be reduced to \bigo{1} and \bigo{n}, respectively, at the expense of reduced security. %\footnoteCC Dumbo-MVBA requires a (\highthreshold)-DKG to achieve said communication complexity. \footnoteDora \textbf{Agreement} These protocols can produce multiple outputs with the specified Validity condition. DORA~\cite{kate2023dora} can produce at least \bigo{n} possible outputs, whereas Abraham \etal and \protocol can produce at most two possible outputs. The external blockchain decides and consumes one of these outputs. In contrast, the other protocols produce only one possible valid output. In the absence of an external blockchain channel, these protocols can be converted to produce one output using \bigo{\log(n)} and \bigo{1} bits of distributed randomness from a DKG setup for DORA and \protocol, respectively.
		}
	\end{flushleft}
\end{table*}


==> tables/smr-related-work.tex <==
% SMR related works table
\begin{tabularx}
	\begin{comment}Proof-of-Work~\cite{nakamoto2008bitcoin}\footnotePredictability
		&
		sync.
		&
		1/2
		&
		\xmark
		&
		\checkmark
		&
		\bigo{\kappa n}
		&
		very high
		&
		\bigo{1}
		&
		CRS
		&
		Hash
	\end{comment}
	\begin{comment}Algorand~\cite{gilad2017algorand}\footnotePredictability
		&
		partial sync.
		&
		1/3
		&
		\xmark
		&
		\checkmark
		&
		\bigo{\kappa cn}\footnoteCommElection
		&
		\bigo{c}
		&
		\bigo{1}
		&
		VRF \& PKI
		&
		VRF
		\\
		BRandPiper~\cite{bhat2021randpiper}
		&
		sync.
		&
		1/2
		&
		\checkmark
		&
		\xmark
		&
		\bigo{\kappa n^3}
		&
		\bigo{n^2}
		&
		\bigo{1}
		&
		SRS \& PKI
		&
		RO \& $q-$SDH
	\end{comment}
\begin{comment}
	OptRand~\cite{bhat2023optrand}
	&
	sync.
	&
	1/2
	&
	\xmark
	&
	\xmark
	&
	\bigo{\kappa n^2}
	&
	\bigo{n}
	&
	\bigo{1}
	&
	SRS \& PKI
	&
	RO \& $q-$SDH
\end{comment}
	\\
	\midrule
	\textbf{SMR Protocol}
	&
	\textbf{Comm. Compl.}
	&
	\textbf{Sign. Compl.}
	&
	\textbf{Exp. Latency RTs}
	&
	\textbf{Setup}
	&
	\textbf{Cryptographic Assumption}
	\\
	\midrule
	HoneyBadgerBFT~\cite{miller2016honey}
	&
	\bigo{n^2B+\kappa n^3}
	&
	\bigo{n^2\log(n)}
	&
	4+4$\log(n)$
	&
	\minthreshold-threshold setup
	&
	Threshold sigs
	\\
	Dumbo 2~\cite{guo2020dumbo}
	&
	\bigo{n^2B+\kappa n^3}
	&
	\bigo{n}
	&
	53
	&
	\highthreshold-threshold setup\footnoteMulWithoutThresh
	&
	Threshold sigs
	\\
	Speeding Dumbo~\cite{guo2022speedingdumbo}
	&
	\bigo{n^2B+\kappa n^3\log(n)}
	&
	\bigo{n}
	&
	16
	&
	\highthreshold-threshold setup\footnoteMulWithoutThresh
	&
	Threshold sigs
	\\
	Dumbo NG~\cite{gao2022dumbong}
	&
	\bigo{n^2B + \kappa n^3 \log(n)}
	&
	\bigo{n}
	&
	16
	&
	\highthreshold-threshold setup\footnoteMulWithoutThresh
	&
	Threshold sigs
	\\
	Narwhal-Tusk~\cite{george2022narwhal}
	&
	\bigo{n^2B + \kappa n^3}
	&
	\bigo{n^2}
	&
	18
	&
	\highthreshold-threshold setup\footnoteMulWithoutThresh
	&
	Threshold sigs
	\\
	WaterBear~\cite{zhang2022waterbear}
	&
	\bigo{\exp(n)}
	&
	0
	&
	\bigo{\exp(n)}
	&
	Auth channels
	&
	None
	\\
	\midrule
	\smrprotocol
	&
	\bigo{n^2B + \kappa n^3 \log(n)}
	&
	0\footnoteReplHash
	&
	22
	&
	Auth channels
	&
	Hash
	\\
	\bottomrule
\end{tabularx}
